Formation and Reconfiguration of Tight Multi-Lane Platoons

Advances in vehicular communication technologies are expected to facilitate cooperative driving. Connected and Automated Vehicles (CAVs) are able to collaboratively plan and execute driving maneuvers by sharing their perceptual knowledge and future plans. In this paper, an architecture for autonomous navigation of tight multi-lane platoons travelling on public roads is presented. Using the proposed approach, CAVs are able to form single or multi-lane platoons of various geometrical configurations. They are able to reshape and adjust their configurations according to changes in the environment. The proposed architecture consists of two main components: an offline motion planner system and an online hierarchical control system. The motion planner uses an optimization-based approach for cooperative formation and reconfiguration in tight spaces. A constrained optimization scheme is used to plan smooth, dynamically feasible and collision-free trajectories for all the vehicles within the platoon. The paper addresses online computation limitations by employing a family of maneuvers precomputed offline and stored on a look-up table on the vehicles. The online hierarchical control system is composed of three levels: a traffic operation system (TOS), a decision-maker, and a path-follower. The TOS determines the desired platoon reconfiguration. The decision-maker checks the feasibility of the reconfiguration plan. The reconfiguration maneuver is executed by a low-level path-following feedback controller in real-time. The effectiveness of the approach is demonstrated through simulations of three case studies: 1) formation reconfiguration 2) obstacle avoidance, and 3) benchmarking against behavior-based planning in which the desired formation is achieved using a sequence of motion primitives. Videos and software can be found online https://github.com/RoyaFiroozi/Centralized-Planning.

==> Sec_extra.tex <==
This paper focuses on motion planning for one and two-dimensional mini platoons. In general, the motion planning algorithms can be classified into three major classes including optimization-based \cite{1428839,article,doi:10.1177/0278364914528132,7535379,Katrakazas_2015}, search-based and sampling-based algorithms. Authors in \cite{20.500.11850/127450,Gonzlez2016ARO} have reviewed and discussed these approaches for autonomous driving applications. Motion planning and navigation in dynamic environment is a challenging problem even for a single vehicle. As the number of vehicles increases, the complexity of the problem increases. Multiple vehicles have to simultaneously interact with the environment as well as other collaborator vehicles.

For highway platooning application, the vehicle's motion is also confined to the road geometry such as lane width or road curvature. Besides highway structure, platoon geometry (longitudinal and lateral inter-vehicle spacing) restricts the motion of the vehicles within the platoon and results in creating a tight environment. Therefore, performing collaborative behaviors in a platoon requires tight navigation of the vehicles. Among all classes of motion planning approaches, optimization-based motion planning is the most effective approach, when tight navigation at high velocity is required.


In most of the studies, a fixed or switching communication graph describes the interconnection structure between the agents. In \cite{1239709} a distributed consensus protocol is introduced by representing the graph structure of the agents as a Laplacian matrix. In \cite{FAX200255}, the eigenvalues of graph Laplacian are used as formation stability criterion.

Morphology control in flocking and particle swarm optimization algorithms is inspired by collective behaviors in nature like birds flock, insects swarm and fish school.

The position of the robot is $q$, the total potential $U(q)$ is the sum of attractive and repulsive potentials and its negative gradient $-\nabla U(q)$ is the local direction of motion of the robot.


In this work we choose matrix $p$ such that all its columns are the same, which means the distance between the vehicles is the same for all the lanes. 

The collaborative maneuvers obtained by motion planning module are computed offline. The family of maneuvers for all the possible configurations are stored on the electronic control unit of the vehicles.


\begin{equation}\label{eq:distance_polytop_feasibility}
\begin{aligned}
&\exists \quad \lambda \succeq 0, \mu \succeq 0, s\\
&\textrm{subject to}
&-b_{1}^{\top} \lambda -b_{2}^{\top} \mu > d_\text{min}\\
& &A_{1}^{\top} \lambda + s = 0\\
& &A_{2}^{\top} \mu - s = 0\\
& &\norm{s} \leq 1.\\
\end{aligned} \end{equation}

\begin{align*}\label{condition}
\dot{y}^i \leq \epsilon_{y},\quad
\dot{\psi}^i \leq \epsilon_{\psi},\quad
v^i = v_{\text{max}},
\end{align*}

\begin{equation*}\label{eq:time_varying_polytope}
\mathcal{P}(z_{k}) = \Bigg\{\begin{bmatrix}
p_{x}\\
p_{y}
\end{bmatrix} \in \mathbb{R}^{2}
\Bigg|A_{k}\begin{bmatrix}
p_{x}\\
p_{y}
\end{bmatrix} \leq b_{k} \Bigg\},
\end{equation*}
where $p_{x}$ and $p_{y}$ are the coordinates of points in two-dimensional space which are representation of the polytope and $A_{k}$ and $b_{k}$ are defined as 
\begin{equation*}\label{eq:polytope_matrices}
A_{k} = 
\begin{bmatrix}
R_k\\
-R_k
\end{bmatrix},\
R_{k} = 
\begin{bmatrix} 
-\sin(\psi_{k})& \cos(\psi_{k})\\
\cos(\psi_{k}) & \sin(\psi_{k}) 
\end{bmatrix},
\end{equation*}
\begin{equation*}
b_{k} = \begin{bmatrix}
\frac{w}{2},
\frac{h}{2},
\frac{w}{2},
\frac{h}{2}
\end{bmatrix}^\top + A_{k}\begin{bmatrix}
x_{k}\\
y_{k}
\end{bmatrix}.
\end{equation*}

\begin{align*}\label{condition}
\dot{y}^i \leq \epsilon_{y},\quad
\dot{\psi}^i \leq \epsilon_{\psi},\quad
v^i = v_{\text{max}},
\end{align*}

\begin{equation}\label{eq:MPC_formulation_reformulated}
\begin{aligned}
% & \underset{{u^i(.|t)},\lambda_{ij}(.|t), \mu_{ij}(.|t), s_{ij}(.|t)}{\text{minimize}}
& \min_{\substack{u^i(\cdot|t),\ \lambda_{ij}(\cdot|t),\\ \mu_{ij}(\cdot|t),\ s_{ij}(\cdot|t)}}
& &\sum_{i=1}^{N_V}\bigg(\sum_{k=t}^{t+N}Q||z^{i}(k|t)-z^{i}_\textrm{Ref}(k|t)||^2_2 \\
& & & +  \sum_{k=t}^{t+N-1}R_1||u^{i}(k|t)||^2_2 + R_2||\Delta u^{i}(k|t)||^2_2\bigg)\\
&\textrm{subject to} & & z^{i}(k+1|t) = f(z^{i}(k|t),u^{i}(k|t)),\\
& & & z^{i}(1|t) = z^{i}(t),\\
& & & z_{\min} \leq z^{i}(k|t) \leq z_{\max},\\
& & & u_{\min} \leq u^{i}(k|t) \leq u_{\max},\\
& & & \bigg(-b_{i}(z^{i}(k|t))^{\top} \lambda_{ij}(k|t) \\
& & & - b_{j}(z^{j}(k|t))^{\top} \mu_{ij}(k|t)\bigg) \geq d_\text{min}\\
& & & A_{i}(z^{i}(k|t))^{\top} \lambda_{ij}(k|t) + s_{ij}(k|t) = 0\\
& & & A_{j}(z^{j}(k|t))^{\top} \mu_{ij}(k|t) - s_{ij}(k|t) = 0\\
& & & \norm{s_{ij}(k|t)} \leq 1\\
& & & -\lambda_{ij}(k|t) \leq 0\\
& & & -\mu_{ij}(k|t) \leq 0\\
& & & i \in \mathcal{V},\ j \in \mathcal{N}_i,\\
\end{aligned} \end{equation}

\begin{figure}
\centering
\includegraphics[scale=0.5]{pics/platoon_conf_set_vertical.PNG}
\caption{(a) 1D platoon: a train-like group of vehicles travelling at close distance $d$ behind each other. (b) 2D platoon in two lanes: The vehicles travel at two lanes. The platoon geometrical pattern is well-defined by parameter vector of $p$ which includes inter-vehicle distance $d$ and shifting distance $d_{\text{shift}}$. This type of configuration facilitates lane change maneuvers. (c) 2D platoon in multiple lanes: Depending on the number of the lanes of the highway, 2D platoons can form configurations on multiple lanes. Yellow arrow denotes horizontal inter-vehicle distance $d$ at each lane and red arrow shows the shifting distance $d_{\text{shift}}$ at each lane.}
\label{fig:platoon_configurations}
\end{figure}

\begin{align}
    h: & \mathbb R^3 \to \mathbb R, \\
    & (x^i(0),v_{\text{max}},T)\mapsto x_{\text{Ref}}^{i},\quad
    \forall{i} \in \mathcal{V}
\end{align}

(b) The polytopic set undergoes affine transformations.

described as the intersection of a set of half-spaces

The paper addresses online computation limitations by employing a family of maneuvers precomputed offline and stored on the vehicles' control units to be executed by a low-level feedback controller in real-time based on the selected desired configuration.

However, MIPs are inherently non-deterministic polynomial time (NP)-complete which in this case scales exponentially with number of the vehicles. 

%%%%%%%%%%%%%%%%%%%%
July4
that captures various pre-identified platoon configurations and reconfiguration maneuvers to transform from one configuration to another. The online hierarchical control system is composed of three levels: traffic operation system (TOS), decision-maker, and path-follower. The top level (TOS) operates in cloud and determines the desired platoon reconfiguration by monitoring the traffic. The decision-maker operates on the platoon leader vehicle. It receives the desire configuration from TOS. Also a copy of the look-up table computed by motion-planner is pre-stored on decision-maker. In addition, the surrounding traffic (outside platoon vehicles) share their future plans with the decision-maker via V2V communication. Using all these information, decision-maker checks whether the desired reconfiguration planned by TOS is feasible or not. If infeasible, it informs TOS to plan a new reconfiguration for future time. If feasible, the maneuver is broadcasted to all the vehicles within the platoon via v2V communication to be executed by a low-level path-following feedback controller in real-time.  
% control units to be executed by a low-level path-following feedback controller in real-time based on the selected desired configuration.
% The output of motion-planner system is a look-up table that captures various pre-identified platoon configurations and reconfiguration maneuvers to transform from one configuration to another.

% The decision-maker selects the desired platoon configuration based on real-time information about the surrounding traffic.

% \item A set of formation patterns also referred to as single-lane and multi-lane platoons is identified and a finite state machine is introduced to capture the transitions between these configurations. Each state of the finite state machine corresponds to a different configuration of the platoon. The decision-maker operates based on the proposed state machine. The continuous maneuvers for transitions among modes are precomputed by motion planner. The guards for switching condition between the modes are defined as a function of the upcoming traffic.

\begin{subequations}\label{eq:path_follower}
\begin{align}
& \min_{\substack{\mathbf{u}(\cdot|t)}}
& &\nonumber{\bigg(\sum_{k=t}^{t+N}||\mathbf{Q}_z^{pf}(\mathbf{z}(k|t)-\mathbf{z}_\textrm{Target}(k|t))||^2_2} \\
& & &+ \nonumber{\sum_{k=t}^{t+N-1}\big(||\mathbf{Q}_{u1}^{pf}(\mathbf{u}(k|t)-\mathbf{u}_\textrm{Target}(k|t))||^2_2}\\
& & &+ \nonumber{||\mathbf{Q}_{u2}^{pf}(\mathbf{u}(k|t))||^2_2 + ||\mathbf{Q}_{\Delta u}^{pf}(\Delta \mathbf{u}(k|t))||^2_2\big)\bigg)}\\
\label{dynamic_path_following}
&\textrm{subject to} & & \mathbf{z}(k+1|t) = f(\mathbf{z}(k|t),\mathbf{u}(k|t)),\\
& & & \mathbf{z}(0|t) = \mathbf{z}(t),\\
& & & \mathbf{z}_{\min} \leq \mathbf{z}(k|t) \leq \mathbf{z}_{\max},\\
& & & \mathbf{u}_{\min} \leq \mathbf{u}(k|t) \leq \mathbf{u}_{\max},\\
\label{input_rate_path_following}
& & & \Delta \mathbf{u}_{\min} \leq \mathbf{u}(k|t)-\mathbf{u}(k-1|t) \leq \Delta \mathbf{u}_{\max},
\end{align} \end{subequations}

, and the input trajectory $\boldsymbol{\tau}_{\mathbf{u}_{\text{Target}}}$ = $\{\mathbf{u}_\textrm{Target}(0), \hdots $, $\mathbf{u}_\textrm{Target}(T)\}$

\begin{table}[]
\caption{Look-up table structure template.}\label{tab:template}
\centering
\begin{tabular}{|c|l|}
\hline
\textbf{Reconfiguration} & \textbf{Trajectories} \\
\hline
\multirow{4}{*}{$(\mathcal{C}_i, \mathcal{C}_f)$} &  $(\boldsymbol{\tau}^i_{z_{\textrm{Target}}}(\rho^i)$, $\boldsymbol{\tau}^i_{u_{\textrm{Target}}}(\rho^i))$\\
& $\rho^i \in (0,1)$,\\
& $\forall i \in$ $\mathcal{V}$\\
\hline
\end{tabular}
\end{table}

and input $\boldsymbol{\tau}^i_{u_{\textrm{Target}}}$ trajectories


\label{obstacle_avoidance_constraint}
& & & \mathcal{P}(\mathbf{z}^{i}(k|t))\cap \mathcal{O}^{r} = \emptyset, \ r \in \mathcal{S},\\





















